HT-Bench: Benchmarking and Learning Dexterous Full-Hand Tactile Representations with Egocentric Vision

Establishing a universal benchmark for tactile representation learning in robotic manipulation remains challenging due to the diversity of tactile sensor designs, data formats, and robot embodiments. Rather than seeking to establish such, we explore a scalable and promising direction for future development: egocentric vision paired with full-hand tactile data. To this end, we introduce \textbf{HT-Bench}, a large-scale multi-task benchmark for dexterous full-hand tactile sensing, comprising 10M RGB frames and 7.8M tactile frames collected across 226 tasks. HT-Bench evaluates tactile representations from three key perspectives: whether they encode meaningful contact geometry, whether they can align tactile observations with visual information, and whether they generalize to unseen tasks. To assess these capabilities, HT-Bench includes four tasks: fine-grained tactile similarity retrieval, masked tactile inpainting, vision-to-tactile synthesis, and multimodal tactile frame prediction. We further propose \textbf{HandTouch}, a vector-quantized vision--tactile encoder that learns tactile representations through progressive spatial, cross-modal, and temporal training. Across HT-Bench, HandTouch consistently outperforms representative tactile encoder baselines, improving Recall@5 on fine-grained tactile similarity retrieval from 74.65\% to 85.23\%, reducing RMSE on masked tactile inpainting from 0.022 to 0.010, and increasing OOD cIoU on vision-to-tactile synthesis from 0.628 to 0.705. These results demonstrate the effectiveness of HandTouch and suggest that large-scale egocentric full-hand tactile data provides a scalable basis for evaluating and advancing tactile representation learning in dexterous manipulation.

==> configs.tex <==
% Common packages
\let\labelindent\relax
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{microtype}
\usepackage{graphicx} \graphicspath{ {figures/} }
\usepackage{amsmath,amssymb}
% ,mathabx,amsbsy,mathtools,etoolbox,mathbbol
\usepackage{times}
\usepackage{graphicx}
\usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\usepackage{acronym}
\usepackage{enumitem}
\usepackage{hyperref}
% \usepackage[breaklinks,colorlinks,linkcolor=red,citecolor=blue]{hyperref}
% \usepackage{balance}
\usepackage{xspace}
\usepackage{setspace}
\usepackage[skip=3pt,font=small]{subcaption}
\usepackage[skip=3pt,font=small]{caption}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage[capitalise,nameinlink]{cleveref}
\usepackage{booktabs,tabularx,colortbl,multirow,multicol,array,makecell}
\usepackage{cuted}
\usepackage{capt-of}
% \usepackage{overpic,wrapfig}
% \usepackage{dblfloatfix}
\usepackage[misc]{ifsym}
\usepackage{pifont}
\usepackage{cite}
\usepackage{listings}
\usepackage{anyfontsize}
\usepackage{tikz}
\usepackage{tcolorbox}


% change the reference style
\renewcommand{\citepunct}{,\penalty\citepunctpenalty\,}
\renewcommand{\citedash}{--}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.6pt] (char) {#1};}}


% draw a frame around given text
\newcommand{\framedtext}[1]{%
\par\vspace{1mm} % Adds space after the box
\noindent\fbox{%
    \parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{#1}%
}%
\par\vspace{2mm} % Adds space after the box
}

\makeatletter
\AddToHook{cmd/appendix/before}{\def\cref@section@alias{appendix}\def\cref@subsection@alias{appendix}}
\makeatother

% \newenvironment{prompt}
% {\begin{tcolorbox}[colback=gray!5,colframe=gray!40,title=Prompt]}
% {\end{tcolorbox}}


% Handy shorthand
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\aka{a.k.a\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% Spacing
% \frenchspacing
% % \medmuskip=2mu   % reduce spacing around binary operators
% % \thickmuskip=3mu % reduce spacing around relational operators
% % \setlength{\abovedisplayskip}{6pt}
% % \setlength{\belowdisplayskip}{6pt}
% % \setlength{\abovecaptionskip}{6pt}
% % \setlength{\belowcaptionskip}{6pt}
% \setlength\floatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\textfloatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\dbltextfloatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\intextsep{0.5\baselineskip plus 3pt minus 2pt}

% Handy math ops
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\kl}{KL}
\newcommand\energy{\mathcal{E}}
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0ex \@plus 0ex \@minus 0ex}{-1em}%
  {\hskip\parindent\normalfont\normalsize\bfseries}%
}
\makeatother

\makeatletter
\AtBeginDocument
 {
   \def\ltx@label#1{\cref@label{#1}}%add braces
   \def\label@in@display@noarg#1{\cref@old@label@in@display{#1}}%remove braces
\def\label@in@mmeasure@noarg#1{%
    \begingroup%
      \measuring@false%
      \cref@old@label@in@display{#1}%remove braces for multline, see https://tex.stackexchange.com/q/737204/2388
    \endgroup}%  
 } %
\makeatother

% Clever references
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\Crefname{figure}{Figure}{Figures}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% Handy Colors
\definecolor{gblue}{HTML}{4285F4}
\definecolor{gred}{HTML}{DB4437}
\definecolor{ggreen}{HTML}{0F9D58}
\def\ra{{\color{gblue}R1}}
\def\rb{{\color{gred}R2}}
\def\rc{{\color{ggreen}R3}}
\definecolor{mygray}{gray}{.92}


% Acronym
\acrodef{dof}[DoF]{Degree of Freedom}
\acrodef{vkc}[VKC]{Virtual Kinematic Chain}
\acrodef{tamp}[TAMP]{Task and Motion Planning}
\acrodef{pddl}[PDDL]{Planning Domain Definition Language}
\acrodef{rddl}[RDDL]{Relational Dynamic Influence Diagram Language}
\acrodef{htn}[HTN]{Hierarchical Task Network}
\acrodef{rrt}[RRT]{Rapidly-exploring Random Tree}
\acrodef{ompl}[OMPL]{Open Motion Planning Library}
\acrodef{iws}[IWS]{Iterated Width Search}
\acrodef{bfs}[BFS]{Breadth First Search}
\acrodef{ai}[AI]{Artificial Intelligence}
\acrodef{spt}[SPT]{Scene Parse Tree}
\acrodef{com}[CoM]{Center of Mass}
\acrodef{mcmc}[MCMC]{Markov Chain Monte Carlo}
\acrodef{ged}[GED]{Graph Editing Distance}
% \acrodef{cg}[$cg$]{\textit{Contact Graph}}
% \acrodef{cg+}[$cg^+$]{\textit{Contact Graph}$^+$}
\acrodef{ga}[GA]{Genetic Algorithm}
\acrodef{sgd}[SGD]{Stochastic Gradient Descent}
\acrodef{llm}[LLM]{Large Language Model}
\acrodef{cg}[$cg$]{contact graph}
\acrodef{cga}[$cg^\oplus$]{augmented contact graph}
\acrodef{sdf}[SDF]{Signed Distance Field}
\acrodef{minlp}[MINLP]{mixed-integer nonlinear program}
\acrodef{cmaes}[CMA-ES]{Covariance Matrix Adaptation Evolution Strategy}
\acrodef{vla}[VLA]{Vision-Language-Action}
\acrodef{vqvae}[VQ-VAE]{Vector Quantized Variational Autoencoder}
\acrodef{vae}[VAE]{Variational Autoencoder}
\acrodef{vbts}[VBTS]{Vision-based Tactile Sensor}
\acrodef{act}[ACT]{Action Chunking with Transformers}

\newcommand{\modelname}{TaF-VLA\xspace}

\newcommand{\revision}[1]{{\color{PineGreen}\emph{#1}}}
